Fine-tuning Large Language Models for Domain-specific Machine Translation

Large language models (LLMs) have shown great potential in domain-specific machine translation (MT). However, one major issue is that LLMs pre-trained on general domain corpus might not generalize well to specific domains due to the lack of domain-specific knowledge. To address this issue, this paper focuses on enhancing the domain-specific MT capability of LLMs, by providing high-quality training datasets and proposing a novel fine-tuning framework denoted by DragFT. DragFT augments LLMs via three techniques: (i) Dictionary-enhanced prompting integrates dictionary information into prompts to improve the translation of domain-specific terminology.; (ii) RAG-based few-shot example selection provides high-quality examples that simulate both the domain and style characteristics; (iii) Fine-tuning with few-shot examples further enhances performance when using in-domain examples. We deploy DragFT on three well-known LLM backbones with 13B training parameters to validate its effectiveness. The results on three domain-specific datasets show that DragFT achieves a significant performance boost and shows superior performance compared to advanced models such as GPT-3.5 and GPT-4o. The drastic performance improvement of DragFT over existing LLMs can be attributed to incorporating relevant knowledge while mitigating noise.

==> tables/RAG.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Use RAG}}  & \multicolumn{3}{c}{\textbf{IT}} & \multicolumn{3}{c}{\textbf{Law}} & \multicolumn{3}{c}{\textbf{Medical}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} 
\small & \small & \small BLEU & \small COMET & \small COMETKiwi& \small BLEU & \small COMET & \small COMETKiwi & \small BLEU & \small COMET & \small COMETKiwi  \\
% \midrule
% \multirow{2}{*}{Dict-Instruct}   & $\times$  &   50.44   &   87.39    &   54.85      &    87.43     &    58.79     &   89.63  \\ 
%    &  $\checkmark$ &   &     &       &       &         &   \\ 
%    \midrule
% \multirow{2}{*}{Dict-Chain}  &  $\times$  & 52.15    &   87.26    &   56.75      &     86.92    &         &     \\ 
%  &  $\checkmark$ &     &      &       &       &         &     \\ 
%  \midrule
% \multirow{2}{*}{Dict-Rephrasing}   & $\times$  &  52.41   &   87.75    &    57.42      &    87.66    &   63.70      &   90.05  \\ 
%  &  $\checkmark$ & \textbf{57.27}  &   \textbf{87.95}  &     60.76     &    88.11    &     70.77    &   90.70  \\

% Dict-Rephrasing+RAG         &   \textbf{57.38}  &   \textbf{87.64}  &          &        &         &     \\ 
\midrule
\multirow{2}{*}{Dict-Instruct}   & $\times$  &   50.44   &   87.39   &   &   54.85      &    87.43   &   &    58.79     &   89.63 & \\ 
   &  $\checkmark$ & 57.18  &  87.90   &       &    59.38   & 88.03  &   & 66.99  &   90.23   &   \\ 
   \midrule
\multirow{2}{*}{Dict-Chain}  &  $\times$  & 52.15    &   87.26   & &   56.75      &     86.92  &  &   64.71      &   90.17 & \\ 
 &  $\checkmark$ & 56.69 &  87.92 &      &  \textbf{62.84} &  \textbf{88.52}  &       &     70.14    & 90.55  &  \\ 
 \midrule
\multirow{2}{*}{Dict-Rephrasing}   & $\times$  &  52.41   &   87.75  &   &    57.42      &    87.66  &   &   63.70      &   90.05  & \\ 
 &  $\checkmark$ & \textbf{57.27}  &   \textbf{87.95}  &   &   60.76    &    88.11  &     &     \textbf{70.77}    &   \textbf{90.70}  & \\

% Dict-Rephrasing+RAG         &   \textbf{57.38}  &   \textbf{87.64}  &     &     &    &    &         &    & \\ 
\bottomrule
\end{tabular}
}
\caption{Ablation study on Tigerbot-13B. The metrics is the average of both zh2en and en2zh.}
\label{table:RAG}
\end{table*}

==> tables/dict.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}   & \multicolumn{3}{c}{\textbf{IT}} & \multicolumn{3}{c}{\textbf{Law}} & \multicolumn{3}{c}{\textbf{Medical}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 
\small  & \small BLEU & \small COMET & \small COMETKiwi& \small BLEU & \small COMET & \small COMETKiwi & \small BLEU & \small COMET & \small COMETKiwi  \\
\midrule
\textbf{Dict-instruction}   &   50.44   &   87.39   &   &   54.85      &    87.43   &   &    58.79     &   89.63 & \\ 

\textbf{Dict-chain}  & 52.15    &   87.26   & &   56.75      &     86.92  &  &   64.71      &   90.17 & \\ 

\textbf{Dict-rephrasing}   &  52.41   &   87.75  &   &    57.42      &    87.66  &   &   63.70      &   90.05  & \\ 
\bottomrule
\end{tabular}
}
\caption{Ablation study on Tigerbot-13B. The metrics is the average of both zh2en and en2zh.}
\label{table:dict}
\end{table*}
